Robust Consistent Video Depth Estimation

We present an algorithm for estimating consistent dense depth maps and camera poses from a monocular video. We integrate a learning-based depth prior, in the form of a convolutional neural network trained for single-image depth estimation, with geometric optimization, to estimate a smooth camera trajectory as well as detailed and stable depth reconstruction. Our algorithm combines two complementary techniques: (1) flexible deformation-splines for low-frequency large-scale alignment and (2) geometry-aware depth filtering for high-frequency alignment of fine depth details. In contrast to prior approaches, our method does not require camera poses as input and achieves robust reconstruction for challenging hand-held cell phone captures containing a significant amount of noise, shake, motion blur, and rolling shutter deformations. Our method quantitatively outperforms state-of-the-arts on the Sintel benchmark for both depth and pose estimations and attains favorable qualitative results across diverse wild datasets.

==> figures/strip.tex <==
\providelength\height%
\setlength\height{8.5cm}%
\providelength\liftup%
\setlength\liftup{-1mm}%

\begin{figure*}[t]
\centering%
%
\jsubfig{\includegraphics[height=\height]{figures/strip/gt.png}}{\vspace{\liftup}(a) Ground truth}%
\hfill%
\jsubfig{\includegraphics[height=\height]{figures/strip/ours.png}}{\vspace{\liftup}(a) Our result}%
\hfill%
\jsubfig{\includegraphics[height=\height]{figures/strip/midas.png}}{\vspace{\liftup}(a) Midas \cite{lasinger2019towards}}%
\hfill%
\jsubfig{\includegraphics[height=\height]{figures/strip/cvd.png}}{\vspace{\liftup}(a) CVD \cite{Luo-VideoDepth-2020}}%
\hfill%
\jsubfig{\includegraphics[height=\height]{figures/strip/colmap.png}}{\vspace{\liftup}(a) COLMAP \cite{schops2017multi}}%
%
\caption{
Strip}
\label{fig:strip}
\end{figure*}


==> table/sintel_pose.tex <==
\begin{table}[ht!]
	\centering
	\caption{ATE RPE on Sintel Clean/Final %\xuejian{add details, mention why there's no colmap/cvd1 comparison}
	}
	\begin{minipage}[b]{0.98\linewidth}
		\centering
        \footnotesize
	   % \setlength{\tabcolsep}{6pt} % Default value: 6pt
        \renewcommand{\arraystretch}{1.2} % Default value: 1
		\begin{tabular}{@{}l ccc}
			\midrule[0.8pt]
			\textbf{Method}  & \textbf{ATE (m)$\downarrow$} & \textbf{RPE Trans (m)$\downarrow$} & \textbf{RPE Rot (deg)$\downarrow$} \\ \midrule[0.8pt]
			DeepV2D & 0.9526 & 0.3819 & 0.1869 \\
            MiDaS-v2 & 0.1883 & 0.0806 & 0.0262\\
			Ours  & \textbf{0.1843}  &  \textbf{0.0723}  & \textbf{0.0095} \\
            \midrule[0.4pt]
			DeepV2D & 0.9192 & 0.5834 & 0.2506 \\
            MiDaS-v2 & 0.2210  &  0.0827  &  0.0258\\
            % \midrule[0.3pt]
			Ours  & \textbf{0.1831}  &  \textbf{0.0714} &  \textbf{0.0088} \\
			\bottomrule[0.8pt]
		\end{tabular}
	\end{minipage}
	\label{tab:sintel_pose}
    % \vspace{-2em}
\end{table}
